Decentralized Planning Using Probabilistic Hyperproperties

Multi-agent planning under stochastic dynamics is usually formalised using decentralized (partially observable) Markov decision processes ( MDPs) and reachability or expected reward specifications. In this paper, we propose a different approach: we use an MDP describing how a single agent operates in an environment and probabilistic hyperproperties to capture desired temporal objectives for a set of decentralized agents operating in the environment. We extend existing approaches for model checking probabilistic hyperproperties to handle temporal formulae relating paths of different agents, thus requiring the self-composition between multiple MDPs. Using several case studies, we demonstrate that our approach provides a flexible and expressive framework to broaden the specification capabilities with respect to existing planning techniques. Additionally, we establish a close connection between a subclass of probabilistic hyperproperties and planning for a particular type of Dec-MDPs, for both of which we show undecidability. This lays the ground for the use of existing decentralized planning tools in the field of probabilistic hyperproperty verification.

==> tables/model-info.tex <==
\begin{table}[t]
\captionsetup{font=small}
\caption{Model info.}
\label{tab:model-info}
\setlength{\tabcolsep}{1pt}
\scalebox{0.9}{
\begin{tabular}{l rrr@{\hskip 12pt}l rrr}
\toprule

experiment & $|\mathcal{M}|$ & $(n,m)$ & bound & experiment & $|\mathcal{M}|$ & $(n,m)$ & bound \\
\midrule

meeting-4x4 & 22 & (2,2) & 0.653 &  meeting-12x7 & 78 & (2,2) & 0.663 \\
meeting-15x9 & 160 & (2,2) & 0.470 & meeting-19x11 & 216 & (2,2) & 0.567 \\

meet-rew-4x4 & 22 & (2,2) & 106.24 & meet-rew-12x7 & 78 & (2,2) & 103.84 \\
meet-rew-15x9 & 160 & (2,2) & 21.43 & meet-rew-19x11 & 216 & (2,2) & 240.28 \\

race-2-4x4 & 18 & (2,2) & 0.798 & race-2-12x7 & 64 & (2,2) & 0.695 \\
race-2-15x9 & 160 & (2,2) & 0.579 & race-2-19x11 & 168 & (2,2) & 0.609 \\

race-3-4x4 & 18 & (3,3) & 0.756 & race-3-12x7 & 64 & (3,3) & 0.614 \\
race-3-15x9 & 160 & (3,3) & 0.392 & race-3-19x11 & 168 & (3,3) & 0.569 \\

opacity-4x4 & 42 & (2,2) & 0.372 & opacity-12x7 & 130 & (2,2) & 0.451 \\
opacity-15x9 & 540 & (2,2) & 0.293 & noninter-4x4  & 22 & (3,4) & 0.708  \\

ISO-4x4 & 22 & (1,2) & 0.467 & ISO-12x7 & 78 & (1,2) & 0.461 \\
ISO-15x9 & 160 & (1,2) & 0.285 & ISO-19x11 & 216 & (1,2) & 0.371 \\

robust-4x4 & 35 & (1,2) & 0.703 & robust-12x7 & 128 & (1,2) & 0.630 \\
robust-15x9 & 640 & (1,2) & 0.586 & robust-19x11 & 203 & (1,2) & 0.728 \\

\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[t]
\captionsetup{font=small}
\caption{Randomized policies.}
\label{tab:random-policies}
\setlength{\tabcolsep}{1pt}
\scalebox{0.9}{
\begin{tabular}{l r@{\hskip 12pt}l r}
\toprule

experiment & random $\pi$ & experiment & random $\pi$ \\
\midrule

meeting-4x4 & 0.098  &  meeting-12x7 & 0.040  \\
meeting-15x9 & 0.002 & meeting-19x11 & 0.008\\

meet-rew-4x4 & 322 & meet-rew-12x7 & 347 \\
meet-rew-15x9 & 42.6 & meet-rew-19x11 & 655 \\

race-2-4x4 & 0.203 & race-2-12x7 & 0.073 \\
race-2-15x9 & 0.018 & race-2-19x11 & 0.009 \\

race-3-4x4 & 0.168 & race-3-12x7 & 0.019 \\
race-3-15x9 & 0.001 & race-3-19x11 & 0.005  \\

opacity-4x4 & 0.001 & opacity-12x7 & 0.002 \\
opacity-15x9 & E-6 & noninter-4x4  & 0.249 \\

ISO-4x4 & 0.013 & ISO-12x7 & 0.013 \\
ISO-15x9 & 0.015 & ISO-19x11 & 0.010 \\

robust-4x4 & 0.226 & robust-12x7 & 0.121 \\
robust-15x9 & 0.044 & robust-19x11 & 0.137 \\

\bottomrule
\end{tabular}
}
\end{table}
